Exotic photonic molecules via Lennard-Jones-like potentials

Ultracold systems offer an unprecedented level of control of interactions between atoms. An important challenge is to achieve a similar level of control of the interactions between photons. Towards this goal, we propose a realization of a novel Lennard-Jones-like potential between photons coupled to the Rydberg states via electromagnetically induced transparency (EIT). This potential is achieved by tuning Rydberg states to a F{\"o}rster resonance with other Rydberg states. We consider few-body problems in 1D and 2D geometries and show the existence of self-bound clusters ("molecules") of photons. We demonstrate that for a few-body problem, the multi-body interactions have a significant impact on the geometry of the molecular ground state. This leads to phenomena without counterparts in conventional systems: For example, three photons in 2D preferentially arrange themselves in a line-configuration rather than in an equilateral-triangle configuration. Our result opens a new avenue for studies of many-body phenomena with strongly interacting photons.

==> commands2018.tex <==

   \setul{0.5ex}{0.1ex}
       \definecolor{Blue}{rgb}{0,0.0,1}
    \setulcolor{Blue}


\newcommand\reduline{\bgroup\markoverwith
{\textcolor{orange}{\rule[-.5ex]{2pt}{0.4pt}}}\ULon}


\newcommand{\out}[1]{\footnote{Outlook: \textcolor{Orange}{#1}}} % openQuestion
\newcommand{\sr}[1]{\reduline{#1}} % keyword
\newcommand{\kw}[1]{\textcolor{Aquamarine}{#1}} % keyword
\newcommand{\oQ}[1]{[openQ]: \textcolor{Bittersweet}{#1}} % openQuestion
\newcommand{\mS}[1]{[mySum]\footnote{ \textcolor{ForestGreen}{#1}} }% my summary
\newcommand{\mQ}[1]{[myQ]: \textcolor{ForestGreen}{#1}} % my question

\renewcommand{\Re}{\mathop{\text{Re}}}
\renewcommand{\Im}{\mathop{\text{Im}}}

%\usepackage[french,polutoniko,greek,polish]{babel}
%\usepackage{polski}
%\newcommand{\cmnt}[1]{[Cmnt: \textcolor{gray}{ #1} ]}
\newcommand{\cmnt}[1]{[Cmnt: \textcolor{gray}{ #1} ]}
\newcommand{\cmntc}[1]{[Cmnt: \textcolor{brown}{ #1} ]}
\newcommand{\todoc}[1]{[TODO: \textcolor{gray}{#1}] }
\newcommand{\todo}[1]{[\textcolor{gray}{\textbf{To do:}}   \textcolor{brown}{#1}]}
\newcommand{\mI}[1]{[myI]: \textcolor{Purple}{#1}} % my question

%\renewcommand{\todoc}[1]{}    \renewcommand{\cmnt}[1]{} 		 \renewcommand{\cmntc}[1]{} % uncomment to not show comments
\newcommand{\rs}{\rm \scriptscriptstyle}
\newcommand{\remove}[1]{}
\newcommand{\meanv}[1]{\left\langle#1\right\rangle}							% <...>
%\def\Om{\Omega\xspace}
\def\om{\omega\xspace}


%\usepackage[round]{natbib}   % omit 'round' option if you prefer square brackets
%\bibliographystyle{plainnat}

\graphicspath{ {./Figures/} }



%%%%%%%%%%%%%%%%%% general commands %%%%%%%%%%%%%%%%%%%%
\newcommand{\blst}{\begin{lstlisting}}
\newcommand{\est}{\end{lstlisting}}

\newcommand{\bit}{ \begin{itemize}{}  }
\newcommand{\eit}{\end{itemize}}

\newcommand{\be}{\begin{enumerate} \itemsep -4pt  }
\newcommand{\ee}{\end{enumerate}}

%\newcommand{\be}{\begin{enumerate}   } %\itemsep -4pt
%\newcommand{\ee}{\end{enumerate}}

\newcommand{\bi}{\begin{itemize}   } %\itemsep -4pt
\newcommand{\ei}{\end{itemize}}

\newcommand{\bma}{\begin{math}} 
\newcommand{\ema}{\end{math}}

\newcommand{\bc}{\begin{columns}} 
\newcommand{\ec}{\end{columns}}
\newcommand{\cl}[1]{\column{#1\textwidth}}  

\newcommand{\bbl}{\begin{block}} 
\newcommand{\ebl}{\end{block}}

\newcommand{\bflsh}{\begin{flashcard}}
\newcommand{\eflsh}{\end{flashcard}}

\newcommand{\bfl}[2]{\begin{flashcard}{#1} {#2} \eflsh}

\newcommand{\beq}{\begin{equation} \vspace{-0em}} 
\newcommand{\eeq}{\vspace{-0.em} \end{equation}}

\newcommand{\beqs}{\begin{equation*}}
\newcommand{\eeqs}{\end{equation*}}

\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}

\newcommand{\beal}{\begin{align}}
\newcommand{\eeal}{\end{align}}

\newcommand{\bvr}{\begin{verbatim}}
\newcommand{\evr}{\end{verbatim}}

%\newcommand{\bflsh}{\begin{lstlisting}}
%\newcommand{\eflsh}{\end{lstlisting}}

\newcommand{\ii}{{\rm i}}						% Imaginary i

\newcommand{\MHz}{\text{MHz}}
\newcommand{\GHz}{\text{GHz}}
\newcommand{\THz}{\text{THz}}
\newcommand{\meV}{\text{meV}}

\newcommand{\tchi}{\ensuremath{\tilde{\chi}}\xspace}
\newcommand{\Gm}{\ensuremath{\Gamma}\xspace}
\newcommand{\GmZ}{\ensuremath{\Gamma^{(0)}}\xspace}
\newcommand{\Om}{\ensuremath{\Omega}\xspace}
%\newcommand{\om}{\ensuremath{\omega}\xspace}
\newcommand{\tGm}{\ensuremath{\tilde{\Gamma}}}
\newcommand{\tGmZ}{\ensuremath{\tilde\Gamma}^{(0)}}
\newcommand{\tG}{\ensuremath{\tilde{G}}\xspace}
\newcommand{\tV}{\ensuremath{\tilde{V}}\xspace}
\newcommand{\tU}{\ensuremath{\tilde{U}}\xspace}

\newcommand{\tm}{\textit{t}-matrix\xspace}

\newcommand{\btGm}{\ensuremath{\tilde{\bf\Gamma}}}
\newcommand{\btGmZ}{\ensuremath{\tilde\bf\Gamma}^{(0)}}
\newcommand{\btG}{\ensuremath{\tilde{\bf G}}}
\newcommand{\btV}{\ensuremath{\tilde{\bf V}}}


\newcommand{\bGm}{\ensuremath{{\bf\Gamma}}\xspace}
\newcommand{\bGmZ}{\ensuremath{{\bf\Gamma}^{(0)}}\xspace}
\newcommand{\bG}{\ensuremath{{\bf G}}\xspace}
\newcommand{\bV}{\ensuremath{{\bf V}}\xspace}


\newcommand{\im}{\item}
\newcommand{\oo}{\item}
\newcommand{\qqq}{\wcc{Q: }}
\newcommand{\aaa}{\wcc{A: }}
\newcommand{\uuu}{\wcc{U: }}
\newcommand{\LLL}{\wcc{L: }}
\newcommand{\lss}{\wcc{Lesson: }}
\newcommand{\rrr}{\wcc{R: }}
\newcommand{\ttt}{\wcc{T: }}
\newcommand{\eee}{\wcc{EXERCISE: \newline}}
\newcommand{\dr}{^{\dagger} }
\newcommand{\drUp}{^{\dagger} }

\newcommand{\se}[1]{\section{#1}}
\newcommand{\sse}[1]{\subsection{#1}}
\newcommand{\ssse}[1]{\subsubsection{#1}}
\newcommand{\sssse}[1]{\subsubsubsection{#1}}
\newcommand{\Ra}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\La}{\Leftarrow}
\newcommand{\ra}{\ensuremath{\rightarrow}\xspace}
\newcommand{\la}{\leftarrow}

\newcommand{\gpe}{Gross-Pitaevskii equation\xspace}
%\newcommand{\bec}{Bose-Einstein condensate\xspace}
\newcommand{\bec}{BEC\xspace}
\newcommand{\becs}{Bose-Einstein condensates\xspace}
\newcommand{\mw}{multi-well\xspace}
\newcommand{\dw}{double-well\xspace}
\newcommand{\tw}{triple-well\xspace}
\newcommand{\bh}{Bose-Hubbard\xspace}

\newcommand{\sst}{\ensuremath{\spadesuit}\xspace}
\newcommand{\cst}{\ensuremath{\clubsuit}\xspace}


\newcommand{\qu}[1]{``#1''}


\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\figref}[1]{FIG.~\ref{#1}}
\newcommand{\al}[1]{\alert{#1}} 
%%%%%%%%%%%%%%%%%% math abbreviations %%%%%%%%%%%%%%%%%%
\newcommand{\bb}[1]{\left(#1\right)}                                		% (..)
\newcommand{\absv}[1]{\left|#1\right|}                             			% |..|
\newcommand{\absvsq}[1]{\absv{#1}^2}	                            		% |..|^2
%\newcommand{\comm}[2]{\left[#1, #2\right]}									% [.., ..]
\newcommand{\braketop}[3]{\left\langle#1\middle|#2\middle|#3\right\rangle}	% <...|...|...>

\newcommand{\hastobe}{\stackrel{!}{=}}                              		% !=
\newcommand{\unit}[1]{\ensuremath{\, \mathrm{#1}}}                     		% unit

%%%%%%%%%% makes problems in the books and I had to comment it! %%%%%%%
%%%\renewcommand{\title}[1]{{\bf {#1}\\}}
%\renewcommand{\author}[1]{{\emph {#1}\newline \newline }}  

%\renewcommand{\vec}[1]{\boldsymbol{#1}}                             % vector
\newcommand{\vecr}{\ensuremath{\vec{r}}\xspace}                     % vector r
\newcommand{\vecrone}{\vec{r_1}}                                    % vector r_1
\newcommand{\vecrtwo}{\vec{r_2}}                                    % vector r_2
\newcommand{\vecmu}{\vec{\mu}}	                                    % vector mu
\newcommand{\veck}{\vec{k}}		                                    % vector k
\newcommand{\vecq}{\vec{q}}		                                    % vector q



\newcommand{\partiald}[1]{\frac{\partial}{\partial #1}}             % d/(d..)
\newcommand{\laplace}{\operatorname{\nabla^2}}                        % laplace

\newcommand{\integralb}[3]{\int\limits_{#1}^{#2} \! \mathrm{d} #3\,} 	% integral
\newcommand{\integral}[1]{\int \! \mathrm{d} #1\,}                    % integral without limits
\newcommand{\integralf}[2]{\int \! \frac{\mathrm{d} #1}{#2}\,}        % integral with a fraction (e.g. int dk/sqrt(2pi))
\newcommand{\intvol}{\integral{^3r}}								% integral over the whole space
\newcommand{\intvolp}{\integral{^3r'}}								% integral over the whole space d^3r'
\newcommand{\intvold}{\intvol\!\intvolp}								% double integral over the whole space d^3r d^3r'

\newcommand{\fourier}[1]{\mathcal{F}\!\left\{#1\right\}}
\newcommand{\invfourier}[1]{\mathcal{F}^{-1}\!\left\{#1\right\}}

\newcommand{\deltaf}{\ensuremath{\operatorname{\delta}}\xspace}	    % delta function
\newcommand{\expf}[1]{\ensuremath{\exp\bb{#1}}\xspace}	    		% exp(...)
\newcommand{\ef}[1]{\ensuremath{\operatorname{e}^{#1}}\xspace}	    % e^(...)

\newcommand{\hamil}{\ensuremath{\operatorname{{\hat{H}}}}\xspace} % Hamilton operator
\newcommand{\hamile}{\ensuremath{\operatorname{{\hat{H}_\text{eff}}}}\xspace} % effective Hamilton operator

\newcommand{\aop}{\ensuremath{\hat{a}^{\phantom\dagger}}\xspace} % annihilation operator
\newcommand{\aopd}{\ensuremath{\hat{a}^\dagger}\xspace} % creation operator
\newcommand{\nop}{\ensuremath{\hat{n}}\xspace} % number operator


\newcommand{\Ns}{\ensuremath{{N_\text{S}}}\xspace}                               % N_s
\newcommand{\Na}{\ensuremath{{N_\text{A}}}\xspace}                               % N_A
\newcommand{\gdd}{\ensuremath{g_\text{dd}}\xspace}                               % g_dd
\newcommand{\add}{\ensuremath{a_\text{dd}}\xspace}                               % a_dd
\newcommand{\aho}{\ensuremath{a_\text{ho}}\xspace} % a_ho
\newcommand{\acrit}{\ensuremath{a_\text{crit}}\xspace}                               % a_crit
\newcommand{\Vdd}{\ensuremath{V_\text{dd}}\xspace}                               % V_dd
\newcommand{\Cdd}{\ensuremath{C_\text{dd}}\xspace}                               % C_dd
\newcommand{\fdip}{\ensuremath{f_\text{dip}}\xspace}                             % f_dip
\newcommand{\Phidd}{\ensuremath{\Phi_\text{dd}}\xspace}                          % Phi_dd
\newcommand{\Vddr}{\ensuremath{V_\text{dd}\bb{\vecr, \vecr'}}\xspace}    		 % V_dd(r, r')
\newcommand{\Vint}{\ensuremath{V_\text{int}(\vecr, \vecr')}\xspace}              % V_int(r, r')
\newcommand{\Eint}{\ensuremath{E_\text{int}}\xspace}                             % E_int
\newcommand{\Eon}{\ensuremath{E_\text{on-site}}\xspace}							 % E_on-site
\newcommand{\mub}{\ensuremath{\mu_\text{B}}\xspace}							 	 % mu_B

\newcommand{\Dx}{\Delta x}
\newcommand{\Dy}{\Delta y}
%\newcommand{\Dz}{\Delta z}
\newcommand{\Dt}{\Delta t}

\newcommand{\PsiOp}{\ensuremath{\operatorname{\hat{\Psi}}}\xspace}

%%%%%%%%%%%%%%%%%% general commands %%%%%%%%%%%%%%%%%%%%
\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}
% \chapterfile is used as a variable
\newcommand{\chapterfile}{}
% command to import one chapter and define the variable \chapterfile
\newcommand{\includechapter}[1]{\label{chap:#1}\renewcommand{\chapterfile}{#1}\input{#1}}
% \igopt[options]{file name}
\newcommand{\igopt}[2][]{\includegraphics[#1]{figures/\chapterfile/#2}}
% \ig[width in units of \textwidth]{file name}
\newcommand{\ig}[2][]{\igopt[width=#1\textwidth]{#2}}
% \figopt[width]{file name}{caption}{placement: h, t, ht, ..}
\newcommand{\figopt}[4][]{
	\begin{figure}[#4]
		\centering
		\ig[#1]{#2}
		\caption{#3}
		\label{fig:#2}
	\end{figure}
}
% \fig[width]{file name}{caption}
\newcommand{\fig}[3][]{
	\figopt[#1]{#2}{#3}{!h} %change fromht to h!
}
% \doublefigopt{width 1}{file name 1}{caption 1}{width 2}{file name 2}{caption 2}{main caption}{placement}
\newcommand{\doublefigopt}[8]{
	 \begin{figure}[#8]
		\centering
		\subfigure[#3]{
			\ig[#1]{#2}
			\label{fig:#2}
		}
		\subfigure[#6]{
			\ig[#4]{#5}
			\label{fig:#5}
		}
		\caption{#7}
		\label{fig:#2_#5}
	\end{figure}
}
% \doublefig{width 1}{file name 1}{caption 1}{width 2}{file name 2}{caption 2}{main caption}
\newcommand{\doublefig}[7]{\doublefigopt{#1}{#2}{#3}{#4}{#5}{#6}{#7}{h!}} %change from ht na h!

\def\up{{\uparrow}}
\def\down{{\downarrow}}
\def\bfu{{\bf f}}
\def\bF{{\bf F}}
\def\bB{{\bf B}}
%\def\bs{{\bf s}}
\def\bS{{\bf S}}
\def\bJ{{\bf J}}
\def\br{{\bf r}}
\def\bd{{\bf d}}
\def\bx{{\bf x}}
\def\by{{\bf y}}
\def\bz{{\bf z}}
\def\bv{{\bf v}}
\def\bk{{\bf k}}
\def\bq{{\bf q}}
\def\bp{{\bf p}}
\def\bP{{\bf P}}
\def\bR{{\bf R}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
%\def\bm{{\bf m}}
\def\bl{{\bf l}}
\def\d{{\rm d}}
\def\Hm{\ensuremath{\mathcal{H}}\xspace}
\def\Am{\ensuremath{\mathcal{A}}\xspace}
\def\e{\ensuremath{\mathcal{E}}\xspace}
\def\Dm{\ensuremath{\mathcal{D}}\xspace}
\def\G{\ensuremath{\mathcal{G}}\xspace}
\def\mV{\ensuremath{\mathcal{V}}\xspace}
\def\p{\ensuremath{\mathcal{P}}\xspace}
\def\m{\ensuremath{\mathcal{M}}\xspace}
\def\s{\ensuremath{\mathcal{S}}\xspace}
%\def\P{\ensuremath{\mathcal{P}}\xspace}
\def\I{\ensuremath{{I}}\xspace}
\def\P{\ensuremath{{P}}\xspace}
\def\E{\ensuremath{\mathcal{E}}\xspace}
\def\B{\ensuremath{\mathcal{B}}\xspace}
\def\Z{\ensuremath{\mathcal{Z}}\xspace}
\def\nn{\nonumber}
\def\s{\ensuremath{\sigma}\xspace}
\def\a{\ensuremath{\alpha}\xspace}
\def\l{\ensuremath{\lambda}\xspace}
\def\ep{\ensuremath{\epsilon}\xspace}
\def\b{\ensuremath{\beta}\xspace}
\def\g{\ensuremath{\gamma}\xspace}
\def\d{\ensuremath{\delta}\xspace}
\def\D{\ensuremath{\Delta}\xspace}
%\def\o{\ensuremath{\omega}\xspace}
%\def\O{\ensuremath{\Omega}\xspace}
\def\eps{\ensuremath{\{eps\}}\xspace}
\def\pmbasis{\ensuremath{\{-,0,+\}}\xspace}

\def\tH{\ensuremath{\tilde{H}}\xspace}

%\newcommand{\rs}{\rm \scriptscriptstyle}

% emphasize/stress
\newcommand{\stress}[1]{\textit{#1}}
\newcommand{\wichtig}[1]{\textit{\textcolor{red}{#1}}}
\newcommand{\wc}[1]{\textit{\textcolor{red}{#1}}}
\newcommand{\wcc}[1]{\textit{\textbf{\textcolor{red}{#1}}}}
\newcommand{\nt}[1]{\textcolor{blue}{\textbf{PB:}} \textit{\textcolor{blue}{#1}}\\}
%\newenvironment{intro}{\itshape}{\normalfont}

%\definecolor{lightgray}{gray}{0.95}
%\definecolor{darkgray}{gray}{0.2}
\newcommand{\todoa}[1]{\vskip0pt\begin{center}\fcolorbox{orange}{white}{\parbox{0.9\textwidth}{\textcolor{blue}{\textbf{To do:}} #1}}\end{center}\vskip0pt}

\newcommand{\eeee}[1]{\vskip1pt\begin{center}\fcolorbox{orange}{white}{\parbox{0.9\textwidth}{\textcolor{blue}{\textbf{Exercise:}} #1}}\end{center}\vskip1pt}


\newcommand{\todob}[1]{\vskip1pt\begin{center}\fcolorbox{black}{lightgray}{\parbox{0.9\columnwidth}{\textcolor{green}{\textbf{To do:}} #1}}\end{center}\vskip1pt}

\newcommand{\takeaway}[1]{\vskip1pt\begin{center}\fcolorbox{black}{pink}{\parbox{0.9\columnwidth}{\textcolor{blue}{\textbf{Takeaway:}} #1}}\end{center}\vskip1pt}

%\newcommand{\qs}[1]{\vskip2pt\begin{center}\fcolorbox{black}{lightgray}{\parbox{0.9\textwidth}{\textcolor{brown}{\textbf{Q:}} #1 \textcolor{brown}{\textbf{?}} }}\end{center}\vskip1pt}

\newcommand{\qs}[1]{\vskip2pt\begin{center}\fcolorbox{green}{white}{\parbox{0.9\textwidth}{\textcolor{brown}{\textbf{Q:}} #1 \textcolor{brown}{\textbf{?}} }}\end{center}\vskip1pt}

\newcommand{\ar}[1]{\vskip2pt\begin{center}\fcolorbox{black}{white}{\parbox{0.9\textwidth}{\textcolor{red}{\textbf{A:}} #1 \textcolor{green}{\textbf{!}} }}\end{center}\vskip1pt}


\newcommand{\bld}[1]{{\textbf{#1}}}

\newcommand{\todocite}[1]{[\textcolor{blue}{\textbf{To do:}} citation missing; #1]}
%\newcommand{\todoc}[1]{[\textcolor{blue}{\textbf{To do:}}  #1]}
%\newcommand{\todopb}[1]{[\textcolor{red}{\textbf{To do:}}  #1]}
%\newcommand{\todopb}[1]{}
%\newcommand{\cmnt}[1]{}
%\newcommand{\cmnt}[1]{\vskip0pt\begin{center}\fcolorbox{blue}{white}{\parbox{0.9\textwidth}{\textcolor{orange}{\textbf{Comment:}} #1}}\end{center}\vskip0pt}
\newcommand{\todoref}[1]{[\textcolor{blue}{\textbf{To do:}} reference missing; #1]}
\newcommand{\revise}[1]{\textcolor{red}{$^\text{revise:}$}\textcolor{darkgray}{\textit{#1}}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}


